Mobile-MMLU: A Mobile Intelligence Language Understanding Benchmark

Rapid advancements in large language models (LLMs) have increased interest in deploying them on mobile devices for on-device AI applications. Mobile users interact differently with LLMs compared to desktop users, creating unique expectations and data biases. Current benchmark datasets primarily target at server and desktop environments, and there is a notable lack of extensive datasets specifically designed for mobile contexts. Additionally, mobile devices face strict limitations in storage and computing resources, constraining model size and capabilities, thus requiring optimized efficiency and prioritized knowledge. To address these challenges, we introduce Mobile-MMLU, a large-scale benchmark dataset tailored for mobile intelligence. It consists of 16,186 questions across 80 mobile-related fields, designed to evaluate LLM performance in realistic mobile scenarios. A challenging subset, Mobile-MMLU-Pro, provides advanced evaluation similar in size to MMLU-Pro but significantly more difficult than our standard full set. Both benchmarks use multiple-choice, order-invariant questions focused on practical mobile interactions, such as recipe suggestions, travel planning, and essential daily tasks. The dataset emphasizes critical mobile-specific metrics like inference latency, energy consumption, memory usage, and response quality, offering comprehensive insights into model performance under mobile constraints. Moreover, it prioritizes privacy and adaptability, assessing models' ability to perform on-device processing, maintain user privacy, and adapt to personalized usage patterns. Mobile-MMLU family offers a standardized framework for developing and comparing mobile-optimized LLMs, enabling advancements in productivity and decision-making within mobile computing environments. Our code and data are available at: https://github.com/VILA-Lab/Mobile-MMLU.

==> Makefile <==
TEX := $(shell git ls-files | grep '\.tex$$')
CLS := $(shell git ls-files | grep '\.cls$$')
STY := $(shell git ls-files | grep '\.sty$$')
MD := $(shell git ls-files | grep '\.md$$' | grep -v README)
ORG := $(shell git ls-files | grep '\.org$$')

MD_TEX := $(patsubst %.md,%.md.tex,$(MD))
ORG_TEX := $(patsubst %.org,%.org.tex,$(ORG))

SED ?= $(shell which gsed 2>/dev/null || which sed)
TAR ?= $(shell which gtar 2>/dev/null || which tar)

OUT ?= .

LATEXMK ?= latexmk
LATEXMK_TEXENGINE ?= xelatex
LATEXMK_OPTS ?= -pdf -$(LATEXMK_TEXENGINE)

MKPDF ?= $(LATEXMK) $(LATEXMK_OPTS)

all: pdf

pdf: xelatex

.PHONY: xelatex
xelatex: LATEXMK_TEXENGINE:=xelatex
xelatex: main

.PHONY: lualatex
lualatex: LATEXMK_TEXENGINE:=lualatex
lualatex: main

.PHONY: pdflatex
pdflatex: LATEXMK_TEXENGINE:=pdflatex
pdflatex: main
	@echo "WARNING: pdfTeX is not supported, only for local preview purposes."
	@echo "         It produces slightly different output than XeTeX, which is used for publishing."

watch: main
	if which inotifywait 2>/dev/null; then \
	  while inotifywait -qe modify $(TEX) $(CLS) $(STY) $(MD) $(ORG); do echo make main; done; \
	else if which fswatch 2>/dev/null; then \
	  fswatch $(TEX) $(CLS) $(STY) $(MD) $(ORG) | (while read; do echo make main; done); \
	fi; else
	  @echo "ERROR: Missing inotifywait (Linux) or fswatch (Mac)."
	fi

main: $(OUT)/main.pdf

$(OUT)/main.pdf: main.tex $(TEX) $(CLS) $(STY) $(MD_TEX) $(ORG_TEX)
	$(MKPDF) $(MKPDF_OPTS) $<

%.md.tex: %.md
	pandoc \
		--from=markdown	\
		--to=latex \
		--biblatex \
		$(if $(shell test -e defaults.yaml && echo 1),--defaults=defaults.yaml,) \
		-o $(patsubst %.md,%.md.tex,$<) \
		$<

%.org.tex: %.org
	pandoc \
		--from=org+citations \
		--to=latex \
		--biblatex \
		$(if $(shell test -e defaults.yaml && echo 1),--defaults=defaults.yaml,) \
		-o $(patsubst %.org,%.org.tex,$<) \
		$<

clean-pandoc:
	rm -f $(MD_TEX) $(ORG_TEX)

clean-latex:
	rm -f $(OUT)/main.{blg,bbl,brf,aux,out,fls,xdv,toc,log,fdb_latexmk,synctex,synctex.gz}

clean-pdf:
	rm -f $(OUT)/main.pdf

clean: clean-pandoc clean-latex clean-pdf

update-bib:
	curl -fLO https://art.anoma.net/art.bib

update-template:
	curl -fsL https://github.com/anoma/art-template/tarball/main \
		| gunzip -c | $(TAR) xv --strip-components=1 \
		--wildcards '*/.gitignore' '*/Makefile' '*/latexmkrc' '*/art.bib' '*/templates' '*/bin'
	git add -f .gitignore Makefile latexmkrc art.bib templates bin

update-template-old: update-template
	bin/fix.sh opts-paper-font main.tex
	bin/fix.sh tabular-center $(TEX)
	test -f art.cls && git rm -f art.cls || true


==> examples/code.tex <==
\section{Source code}

{\small
\begin{minted}{python}
def even_constraint(last_state, next_state_var, solver):
    n = solver.IntVar(0, solver.infinity(), 'n_even')
    b = solver.BoolVar('b_even')
    solver.Add(next_state_var - 2 * n <= M * (1 - b))
    solver.Add(next_state_var - 2 * n >= -M * (1 - b))
    return [(b, 1)]
\end{minted}
}

\begin{betterpython}
def even_constraint(last_state, next_state_var, solver):
    n = solver.IntVar(0, solver.infinity(), 'n_even')
    b = solver.BoolVar('b_even')
    solver.Add(next_state_var - 2 * n <= M * (1 - b))
    solver.Add(next_state_var - 2 * n >= -M * (1 - b))
    return [(b, 1)]
\end{betterpython}

\begin{lstlisting}{python}
def odd_constraint(last_state, next_state_var, solver):
    n = solver.IntVar(0, solver.infinity(), 'n_odd')
    b = solver.BoolVar('b_odd')
    solver.Add(next_state_var - 2 * n - 1 <= M * (1 - b))
    solver.Add(next_state_var - 2 * n - 1 >= -M * (1 - b))
    return [(b, 1)]
\end{lstlisting}


==> examples/test.tex <==
\section{Text}

Regular text.?! 0-123+456*789/0

\texttt{ Monospace text.?! 0-123+456*789/0!}

\textit{ Italic text.?! 0-123+456*789/0!}

\textbf{ Bold text.?! 0-123+456*789/0!}

\section{Math Equations}\label{math-equations}

You may want to display math equations in three distinct styles: inline,
numbered or non-numbered display. Each of the three are discussed in the next
sections.

\subsection{Inline (In-text) Equations}\label{inline-in-text-equations}

A formula that appears in the running text is called an inline or in-text
formula. It is produced by the \textbf{math} environment, which can be invoked
with the usual \texttt{\textbackslash{}begin,\ ...\ \textbackslash{}end}
construction or with the short form \texttt{\textbackslash{}\$\ ...\
\textbackslash{}\$}. You can use any of the symbols and structures, from
\(\alpha\) to \(\omega\), this section will simply show a few examples of
in-text equations in context. Notice how this equation: \(\lim_{n\rightarrow
\infty}x=0\), set here in in-line math style, looks slightly different when set
in display style. (See next section).

\subsection{Display Equations}\label{display-equations}

A numbered display equation---one set off by vertical space from the text and
centered horizontally---is produced by the \textbf{equation} environment. The
\textbf{displaymath} environment produces an unnumbered display equation.

Again, in either environment, you can use any of the symbols and structures
available in \LaTeX@; this section will just give a couple of examples of
display equations in context. First, consider Equation~\ref{eq-oneequation},
shown as an inline equation above:

\begin{equation}\phantomsection{
\lim_{n\rightarrow \infty}x=0
}\label{eq-oneequation}\end{equation}

Notice how it is formatted somewhat differently in the \texttt{displaymath}
environment. Now, we'll enter an unnumbered equation:

\[\sum_{i=0}^{\infty} x + 1\]

Note some fine points concerning \texttt{mathit} and how math and text fonts are
different sometimes.

\begin{center}
  \begin{tabular}[c]{|l|l|l|l|}
    just math & $brown~fox$ \\
    \texttt{mathit} & $\mathit{brown~fox}$ \\
    \texttt{textit} & $\textit{brown~fox}$ \\
    \texttt{textbf}& \textbf{brown~fox} \\
    \texttt{mathbf}& $\mathbf{brown~fox}$ \\
    \texttt{mathrm}& $\mathrm{brown~fox}$ \\
    \texttt{textrm}& \textrm{brown~fox} \\
    \texttt{boldsymbol}& $\boldsymbol{brown~fox}$ &
    $\boldsymbol{\partial\times\sum_i}$\\
              && $\partial\times\sum_i$&just math \\
    text mono spaced& s\texttt{st}t &\\
    math mono spaced& $\mathrm{s}\mathtt{st}\mathrm{t}$&
  \end{tabular}
\end{center}

\subsubsection{More information}

A numbered display equation---one set off by vertical space from the text and
centered horizontally---is produced by the \textbf{equation} environment. An
unnumbered display equation is produced by the \textbf{displaymath} environment.

\paragraph{Further details}

Again, in either environment, you can use any of the symbols and structures
available in \LaTeX@; this section will just give a couple of examples of
display equations in context. First, consider ~\eqref{eq-oneequation}, shown as
an inline equation above:

\section{Math Tests}

\begin{definition}[name={Heterogeneous Validity \protect\citep{art-2024-heterogeneous-paxos-20-specs}}, label={def:het-valid}]
    A consensus execution\todo{take Guerraoui definition for what an execution
    is} is \emph{valid} if all decided values were proposed in that execution. A
    consensus protocol is \emph{valid} if all possible executions are valid.
\end{definition}

Characterization of the Imaginary Forms Theorem. Let $S=\left\{v_1, v_2, \ldots,
v_k\right\}$ be a set of vectors in $\mathbb{R}^n$.

% \begin{center} |"|πκομπ̈ρέσα, αντιανταντ ̈ ικός, ελεγκ ̈ τής \end{center}

\begin{center}
    $\perp$
    \begin{equation}
        \begin{split}
        &(\mathit{Blue}, \mathit{Red})\\
        &\mathcal{ABC DEF GHI JKL MNO PQR ST UVW XYZ}\\
        &\mathbb{ABC DEF GHI JKL MNO PQR ST UVW XYZ}\\
        &\mathfrak{ABC DEF GHI JKL MNO PQR ST UVW XYZ}\\
        &\mathscr{ABC DEF GHI JKL MNO PQR ST UVW XYZ}\\
        \end{split}
    \end{equation}
\end{center}
%\renewcommand{\operatorname}[1]{\mathop{\text{#1}}}
Consider $\mathcal{F}(S)=\sum_{i=1}^k \delta\left(v_i v_j w\right) \sigma_{i,
j}$. If $\mathcal{F}(S) \leq \varepsilon$, then
$$
\phi(S, \alpha)=\frac{1}{2 \pi i} \int_{-\infty}^{753} \frac{\tilde{W}_n(\gamma) \cos \left(\sqrt{x^2}\right)}{f^{\prime}(x) R / a} d x=\operatorname{det}\left(\begin{array}{cc}
\alpha^2 & \Pi \\
\omega & x \otimes y
\end{array}\right)
$$

\begin{remark}
    If $\beta \in \Gamma$, then the form is undefined at the points in $S \cap
    \Gamma$, and the integral $l_l\left(i_1\right)$ diverges as $\varepsilon
    \rightarrow 0$. This pathological behavior can be handled by taking $\Gamma
    \subseteq S$.
\end{remark}

Graph three coloring is a common example used to introduce CSPs to new
audiences. The goal is to color the nodes of a graph with three colors such that
no two same-colored nodes touch. 

\begin{equation}
    \forall c \in C, t \in E_{G, c}, \quad \prod_{i<a(c)} f_V(t_i) \in E_{H, c}.    
\end{equation}


\begin{equation}
    \sum_{i=0}^\infty c \in C, t \in E_{G, c}, \quad \int_{i<a(c)} f_V(t_i) \in E_{H, c}.    
\end{equation}

The CSP itself consists of a single binary relation asserting the inequality
between three elements, typically named after primary colors.

\begin{equation}\label{equation:three-color-neq-def}
  \neq\ = \{ (\mathit{Blue}, \mathit{Red}), (\mathit{Blue}, \mathit{Green}), (\mathit{Red}, \mathit{Blue}), (\mathit{Red}, \mathit{Green}), (\mathit{Green}, \mathit{Blue}) \}
\end{equation}

Graphs become instances by translating edges into binary relations. Take this
graph as an example;

\begin{center}
\begin{tikzpicture}[thick]
  \node (A) at (0,0) {$x_1$}; \node (B) at (2,0) {$x_2$}; \node (C) at (4,0)
  {$x_3$}; \node (D) at (1,-2) {$x_4$}; \node (E) at (3,-2) {$x_5$};

  \draw (A) -- (B) -- (C); \draw (A) -- (D) -- (E) -- (C); \draw (D) -- (B);
  \draw (E) -- (B);
\end{tikzpicture}
\end{center}

\subsection{Corresponding CSP instance}

We can simply list the edges using the inequality relation to produce the
corresponding CSP instance;

\begin{equation}
    x_1 \neq x_2 \wedge x_1 \neq x_4 \wedge x_2 \neq x_3 \wedge x_2 \neq x_4 \wedge x_2 \neq x_5 \wedge x_3 \neq x_5 \wedge x_4 \neq x_5
\end{equation}

A solution to the graph coloring problem is then an assignment of colors that
satisfies the instance. 


\begin{table*}[!h]
\begin{center}
\begin{tabular}{p{1.5cm}p{13cm}}
\toprule
  \textbf{Role} & \textbf{Description} \\
\midrule
  Authorizer & approves the resource consumption on the application level. The
  resource logic encodes the mechanism that connects the authorizer's external
  identity (public key) to the decision-making process \\
  Annuler & knows the data required to nullify a resource \\
  Creator & creates the resource and shares the data with the receiver \\
  Owner & can both authorize and annul a resource \\
  Sender & owns the resources that were consumed to create the created resource
  \\
  Receiver & owns the created resource \\
\bottomrule
\end{tabular}
\caption{Resource-related roles.}
\end{center}
\end{table*}


If we think about the structure of this graph, we notice that it has three
triangles, the left and right side triangles $(x_1, x_2, x_4)$  and $(x_2, x_3,
x_5)$, and the central triangle $(x_2, x_4, x_5)$. Each must be a triple of
distinctly colored points. The edge between $x_4$ and $x_5$ forces those two to
have distinct colors, while the two side triangles share a color at $x_2$. These
two observations force us to conclude that the left triangle has the colors of
the right triangle flipped along the bisector going through $x_2$. If we
arbitrarily select $x_1$ to be $\mathit{Blue}$ and $x_2$ to be $\mathit{Red}$,
we are then forced into the coloring;

\begin{equation}
 \langle x_1 \rightarrow \mathit{Blue}; x_2 \rightarrow \mathit{Red}; x_3 \rightarrow \mathit{Green}; x_4 \rightarrow \mathit{Green}; x_5 \rightarrow \mathit{Blue}\rangle,
\end{equation}

which will satisfy this instance. We can place these colors back on the graph to
verify the solution visually.

Citations are also possible, for example: \citep{christopher_goes_2023_8279842}


==> templates/pandoc.tex <==
\let\autocite=\citep

\providecommand{\tightlist}{%
  \setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}

